Asymmetry in Low-Rank Adapters of Foundation Models

Parameter-efficient fine-tuning optimizes large, pre-trained foundation models by updating a subset of parameters; in this class, Low-Rank Adaptation (LoRA) is particularly effective. Inspired by an effort to investigate the different roles of LoRA matrices during fine-tuning, this paper characterizes and leverages unexpected asymmetry in the importance of low-rank adapter matrices. Specifically, when updating the parameter matrices of a neural network by adding a product $BA$, we observe that the $B$ and $A$ matrices have distinct functions: $A$ extracts features from the input, while $B$ uses these features to create the desired output. Based on this observation, we demonstrate that fine-tuning $B$ is inherently more effective than fine-tuning $A$, and that a random untrained $A$ should perform nearly as well as a fine-tuned one. Using an information-theoretic lens, we also bound the generalization of low-rank adapters, showing that the parameter savings of exclusively training $B$ improves the bound. We support our conclusions with experiments on RoBERTa, BART-Large, LLaMA-2, and ViTs.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section_04_theory.tex <==
\section{Theoretical Analysis}
\label{sec:Analysis}

In this section, we analyze the asymmetry in prediction tasks and its effect on generalization. We discuss a general case rather than a specific neural network architecture, considering rank $r$ adaptation of any parameter matrix $W = W_0 + B A$ used multiplicatively on some input-dependent vector, i.e.,
\begin{equation}
%\resizebox{0.4\textwidth}{!}{$
\mathrm{layerOutput} = \psi((W_0 + BA) \cdot \phi(\mathrm{layerInput}), \dots)
%$}
\label{eq:Lora}
\end{equation}
for some differentiable functions $\psi, \phi$. Here, $\psi$ may take more arguments depending on $\mathrm{layerInput}$, which  may have their own low rank adapted parameter matrices.  This generic form encompasses both feedforward and attention layers. 

%Note that (a) neural networks are evaluated on the correctness of their outputs\justin{not sure what this means or why it's relevant}. and (b) 
In this setting, $A$ serves to extract $r$ features from $\phi(\mathrm{layerInput})$, which are then used by $B$ to predict some desired output for future layers.  We will argue that training $B$ to predict the output is crucial for correct outputs, while using a random $A$ is often sufficient, as $B$ can be optimized to use whatever information is retained in the $r$-dimensional projection $A\cdot\phi(\mathrm{layerInput})$.

\subsection{$A$, $B$ asymmetry in prediction tasks}

If we wish to reduce the effort of training both $A$ and $B$ in \eqref{eq:Lora}, in principle either $A$ could be frozen and $B$ tuned or $B$ frozen and $A$ tuned. As shown in \S\ref{sec:exps} and elsewhere, these two options are not empirically equivalent: It is best to freeze $A$ and tune $B$. In this section, we seek to understand the principle behind this asymmetry by theoretically analyzing the fine-tuning of a class of prediction models. We first build intuition with least-squares linear regression.

%\rickard{I think we don't really know what's best in terms of generalization versus ability to fit the data? The empirical evidence suggests mostly that the asymmetry comes from ability to fit the training data rather than generalization error?}\kristjan{Yep, this section is talking about ability to fit, not gen err}

\subsubsection{Multivariate linear least-squares}\label{sec:linear}

 As a simple example analogous to a single network layer, we study $d_{in}$-to-$d_{out}$ least-squares linear regression (in \eqref{eq:Lora}, set $\phi$, $\psi$ to be identity). Specifically, suppose there is an input $X \in \mathbb{R}^{d_{in}}$, an output $Y \in \mathbb{R}^{d_{out}}$, and a pre-trained linear model 
\[
y_{pre}(X) = W_0 X + b_0,
\]
where $W_0 \in \mathbb{R}^{d_{out} \times d_{in}}$ and $b_0 \in \mathbb{R}^{d_{out}}$. 
With this model held constant, our goal is regressing $(Y_{targ},X_{targ})$ pairs where $Y_{targ}$ is given by:
\begin{align*}
&Y_{targ} = W_{targ} X_{targ} + b_{targ} 
\end{align*}
with $W_{targ} = W_0 + \Delta$. Following LoRA, we model the target $\Delta$ using a low rank update to the pre-trained $W_0$, i.e. $W = W_0 + BA$: 
\[
\hat{y}(x) = (W_0 + BA) x + b,
\]
where $B \in \mathbb{R}^{d_{out} \times r}$ and $A \in \mathbb{R}^{r \times d_{in} }$ for some $r$. 

To find an $A$ and $B$ that best matches the output, we optimize the least squares loss on the difference between $\hat{y}$ and $Y_{targ}$:
\begin{equation}
%\resizebox{0.4\textwidth}{!}{
%$
\mathcal{L}(A,B) \!=\! \mathbb{E}_{(Y_{targ}, X_{targ})} [\left\| Y_{targ} \!-\! (W_0 \!+\! BA) X_{targ} \!-\! b\right\|_2^2].
%$
%}
\label{eq:L2loss}
\end{equation}
%

Below, we present lemmas on minimizing this loss while freezing either $A$ or $B$. In both, for simplicity, we set $b = b_{targ}$ and $\mathbb{E}[X_{targ}] = 0$ and defer proofs to Appendix \ref{app:LS}.
\begin{lemma}[Freezing $A$ yields regression on projected \textbf{features}]
    \label{thm:A_L2}
    Optimizing $\mathcal{L}(A,B)$ while fixing $A = Q$ with $Q Q^\top = I_r$ yields %is equivalent to ordinary least squares regression problem mapping $Q X_{targ}$ to $(Y_{targ} - W_0 X_{targ})$, yielding
    \[
        B^\ast = \Delta \Sigma Q^\top  (Q \Sigma Q^\top )^{-1},
    \]
    where $\Sigma = \mathrm{Cov}[ X_{targ} ]$, with expected loss 
    \begin{align*}
 \mathcal{L}(Q,B^{\ast})  =\ &d_{out} \sigma^2 + \mathrm{Tr}[\Delta \Sigma \Delta^\top ] \\&- 
 \mathrm{Tr} [Q \Sigma \Delta^\top  \Delta \Sigma Q^\top  (Q \Sigma Q^\top )^{-1}].
\end{align*}
\end{lemma}
\begin{lemma}[Freezing $B$ yields regression on projected \textbf{outputs}]
\label{thm:B_L2}
    Optimizing $\mathcal{L}(A,B)$ while fixing $B = U$ with $U^\top U = I_r$ %is equivalent to ordinary least squares regression problem mapping $X_{targ}$ to $U^\top (Y_{targ} - W_0 X_{targ})$, yielding 
    yields
    \[
    A^\ast = U^\top  (W_{targ} - W_0),
    \]
    %The expected squared prediction error is 
    with expected loss
    \begin{align*}
    \mathcal{L}(A^\ast,U) = d_{out} \sigma^2 + \mathrm{Tr}[\Delta \Sigma \Delta^\top ] - \mathrm{Tr}[U^\top  \Delta \Sigma \Delta^\top  U],
\end{align*}
where $\Sigma = \mathrm{Cov}[ X_{targ} ]$.
\end{lemma}
Comparing the lemmas above, $A^\ast$ is simply the $U$ projection of the targeted change in weight matrix $\Delta = W_{targ} - W_0$. Unlike $B^\ast$, the optimal choice of $A^\ast$ does not consider the input data distribution captured by $\Sigma$. 

Intuitively, if the goal of adaptation is to approximate some desired output, then projecting away the majority (since $r \ll d_{out}$) of the output is undesirable.  
%
In contrast, projecting away a portion of the input feature space will be less damaging, if the information $X_{targ}$ contains about $Y_{targ}$ is redundant (c.f., neuron dropout \citep{srivastava2014dropout} in neural network training) or if the distribution of $X_{targ}$ tends to be low-rank. 

Consider the following extreme example. If $\Sigma = F F^\top $ is at most rank $r$, e.g.\ if $F\in {d_{in} \times r}$, then for each $X$ there exists\footnote{Here $F^{\dag}$ denotes pseudoinverse.} an $N = F^{\dag} X\in \mathbb{R}^r$ such that $X = F N$. Suppose you have tuned a pair $A_\ast$, $B_\ast$. For any orthonormal $Q\in\mathbb{R}^{r \times d_{in}}$ (e.g. one drawn at random), we can write
\begin{align*}
    B_\ast A_\ast X &= B_\ast A_\ast F N \\
    %&= B_\ast A_\ast F ((QF)^{-1} QF) N \\
    &= (B_\ast A_\ast F (QF)^{-1}) Q X,
\end{align*}
i.e. regardless of $A_\ast$, $B_\ast$, for any (random) $Q$, there is an exactly equivalent LoRA adaptation with $A = Q$ and $B = (B_\ast A_\ast F (QF)^{-1})$.
 In this setting, therefore, randomizing $A$ (to $Q$) is equally expressive to tuning it (using $A_\ast$). 

% \paragraph{Comparing the two options - intuition} Consider the extreme example of $r = 1$. Then for freezing $B$, the predicted output $\hat{y}$ must be proportional to the random $B$. Since $B$ is not tuned to the data, this random vector is unlikely to be an effective basis for predicted $\hat{y}$, particularly if the covariance of the true $Y$ has low effective rank. For freezing $A$, on the other hand, $B$ is free to be tuned to use the random feature $A X$ to best predict $Y$, taking into account the dominant directions of variation implied by the covariance of $Y$. 

This intuition is also reflected in the typical LoRA initialization. When doing full LoRA (tuning both $A,B$), $A$ usually is initialized to a random Gaussian matrix, and $B$ is initialized to zero. This procedure---presumably empirically derived by \citet{Hu2021LoRALA}---intuitively fits our analysis above, since random $A$ yields good random predictive features, in contrast to using a random output prediction basis. Initializing $B$ to zero then starts the optimization at a zero perturbation of the pretrained model. 

We validate the above intuition with the following theorem:
\begin{theorem}[$A$, $B$ output fit asymmetry]
\label{thm:ABcomp}
Consider the settings of Lemmas \ref{thm:A_L2} and \ref{thm:B_L2}, and suppose $U, Q$ are sampled uniformly from their respective Stiefel manifolds. Then, 
%\[
$
\mathcal{L}(A^\ast, U) \geq \mathcal{L}(Q, B^\ast)
%\]
$
with high probability as $\nicefrac dr \rightarrow \infty$.
\end{theorem}
In other words, the least-squares prediction loss of only fine-tuning $B$ is at least as good as only fine-tuning $A$. 

\textbf{Intuition on asymmetry gap.} Theorem \ref{thm:ABcomp} is built on the following inequality:
\begin{align}
\mathrm{Tr}[&\Sigma Q^\top  (Q \Sigma Q^\top )^{-1} Q \Sigma \Delta^\top  \Delta] \nonumber\\&\geq \mathrm{Tr}[(Q^\top  Q) \Sigma Q^\top  (Q \Sigma Q^\top )^{-1} Q \Sigma \Delta^\top  \Delta].
\label{eq:ineq}
\end{align}
%Note that $\Sigma Q^\top  (Q \Sigma Q^\top )^{-1} Q \Sigma \Delta^\top  \Delta$ is rank $r$.
Let us consider an example regime to build intuition on the size of this gap. Following intuition that freezing $A$ is most successful when the information content of the input is redundant (c.f., \citet{Aghajanyan_2021_intrinsic}), suppose the distribution of $X$ is low rank, i.e., $\Sigma$ is of rank $r_X$. We can then write $\Sigma = U_X S_X U_X^\top $, where $U_X\in \mathbb{R}^{d_{in} \times r_X}$ is orthogonal and $S_X \in \mathbb{R}^{r_X \times r_X}$ is diagonal with nonnegative real entries.

For intuition, set $r_X = r$ and $S_X = \sigma^2 I_{r}$. We then have % and $\Delta = \delta I$ 
\begin{align*}
%&
\Sigma Q^\top  (Q \Sigma Q^\top )^{-1} Q \Sigma \Delta^\top  \Delta %\\&= \sigma^2  U_X  U_X^\top  Q^\top  (Q U_X  U_X^\top  Q^\top )^{-1} Q U_X U_X^\top  \Delta^\top  \Delta\\&
= \sigma^2 U_X U_X^\top  \Delta^\top  \Delta,
\end{align*}
which no longer depends on $Q$. The expectation of the key inequality gap in \eqref{eq:ineq} then becomes 
\begin{align*}
    &\mathbb{E}_Q\mathrm{Tr}[\Sigma Q^\top  (Q \Sigma Q^\top )^{-1} Q \Sigma \Delta^\top  \Delta]\\
    &- \mathbb{E}_Q\mathrm{Tr}[(Q^\top  Q) \Sigma Q^\top  (Q \Sigma Q^\top )^{-1} Q \Sigma \Delta^\top  \Delta]\\
    &= \mathbb{E}_Q\mathrm{Tr}[(I - Q^\top  Q)\sigma^2 U_X U_X^\top  \Delta^\top  \Delta ]\\
    &\rightarrow \left(1 - \frac{r}{d}\right) \mathrm{Tr}[U_X U_X^\top  \Delta^\top  \Delta]
\end{align*}
as $d$ becomes large. In other words, the performance advantage of tuning $B$ over $A$ is large when $d \gg r$, which is the typical regime in practice.

%\paragraph{Example: Isotropic input distribution, low rank $\Delta$}
%Consider the setting that the input distribution is isotropic, i.e. $\Sigma = \sigma^2 I_{d_{in}}$. 
% Then \eqref{eq:ineq} simplifies to
% \begin{align*}
%     &\mathrm{Tr}[\Sigma Q^\top  (Q \Sigma Q^\top )^{-1} Q \Sigma \Delta^\top  \Delta] \\&\geq \mathrm{Tr}[(Q^\top  Q) \Sigma Q^\top  (Q \Sigma Q^\top )^{-1} Q \Sigma \Delta^\top  \Delta].
% \end{align*}



% As an example, suppose its nonzero eigenvalues\footnote{These are real and positive.} are all equal to some value $\tau$. Then 
% \[
% \mathbb{E}_{Q}\mathrm{Tr}[(Q^\top  Q) \Sigma Q^\top  (Q \Sigma Q^\top )^{-1} Q \Sigma \Delta^\top  \Delta] \rightarrow \tau \frac{r^2}{d} \ll \tau r
% \]
% when $d \gg r$, implying the potential for a significant asymmetry gap in terms of ability to fit the output.







% \paragraph{Low rank interpretation}
% Note that the inequality in the bounding of $III_A$ above arises from the fact that $Q Q^\top  \Sigma$ projects $\Sigma$ down to a lower, random subspace. This contraction (and hence the gap between $III_A$ and $III_B$) will be most significant (in expectation) when the dimensionality $d_{in}$ is large relative to $r$ and the eigenvalues of $\Sigma$ are concentrated, i.e. $\Sigma$ is dominated by a low-rank component. 

%Consider the following extreme example. If $\Sigma = F F^\top $ is rank $r$ or less, i.e. $F\in {d_{in} \times r}$, then, $X = F N$ for some random vector $N \in \mathbb{R}^r$, and $B A X = B A F N = (BAF (QF)^{-1}) UF N = (BAF (QF)^{-1}) Q X = B' Q X $, i.e. setting $A$ to be random loses no expressive power vs. tuning it.






% \subsection{Theory: logistic regression}

% \paragraph{Setting.} Training dataset $\{(x_i, y_i)\}_{i=1}^n$ where $x_i \in \R^{d}$ (features) and $y_i \in \{1, \dots, K\}$ (label). Denote by $e_i \in \R^{K}$ s.t. $e_{ii} = 1$, $e_{ik} = 0$ for $k \neq i$. The log likelihood is given by the cross-entropy error function, i.e.,
% \begin{equation} \label{eq:logreg_lkl}
%     \mathcal{L}(w_1, \dots, w_K) = \sum_{i=1}^n \sum_{k=1}^K e_{y_i, k} \ln(p_{i,k})
% \end{equation}
% where $p_{i,k} = \frac{\exp(w_k^\top  x_i)}{\sum_{l=1}^K \exp(w_l^\top  x_i)}$ and $w_k \in \R^d$. 

% Let $W \in \R^{K \times d}$ s.t. the $k$-th row of $W$ is $w_k$. Then, \eqref{eq:logreg_lkl} can be written as
% \begin{equation} \label{eq:logreg_lkl_2}
%     \mathcal{L}(W) = \sum_{i=1}^n e_{y_i}^\top  \ln\left(\frac{e^{W x_i}}{\mathbf{1}^\top  e^{W x_i}}\right) \,,
% \end{equation}
% where $\mathbf{1}$ is the column vector of size $K$ with all elements equal to 1. Maximum likelihood estimation aims at maximizing \eqref{eq:logreg_lkl_2} over $W$. The gradient of \eqref{eq:logreg_lkl_2} w.r.t. $W$ is
% \begin{equation}
%     \nabla_W  \mathcal{L}(W) = \sum_{i=1}^n (e_{y_i} - p_i(W)) x_i^\top  \,,
% \end{equation}
% with $p_i(W) =  \frac{e^{W x_i}}{\mathbf{1}^\top  e^{W x_i}} \in \R^K$.

% Now, assume $W = W_0 +\Delta W = W_0 + BA$ with $B \in \R^{K \times r}$, $A \in \R^{r \times d}$, $r < \min(d, K)$.

% \paragraph{Freezing $B = U$.} Assume $B$ is frozen to $U$ s.t. $U^\top  U = I_r$ and only $A$ is trained. The gradient of the log likelihood \eqref{eq:logreg_lkl_2} w.r.t $A$ is
% \begin{equation}
%     \nabla_A  \mathcal{L}(UA) = U^\top  \sum_{i=1}^n (e_{y_i} - p_i(UA)) x_i^\top 
% \end{equation}

% \paragraph{Freezing $A = Q$.} Assume $A$ is frozen to $Q$ s.t. $Q Q^\top  = I_r$ and only $B$ is trained. The gradient of the log likelihood \eqref{eq:logreg_lkl_2} w.r.t $B$ is
% \begin{equation}
%     \nabla_B  \mathcal{L}(BQ) = \sum_{i=1}^n (e_{y_i} - p_i(BQ)) (Q x_i)^\top 
% \end{equation}
% Freezing $A=Q$ is then equivalent to performing logistic regression on the training dataset with features projected by $Q$: $\{(Qx_i, y_i)\}_{i=1}^n$.

% \paragraph{Comparison.}

\subsubsection{Nonlinear losses and multilayer models}
Recalling \eqref{eq:Lora} with an input transformation $\phi$ and output transformation $\psi$, consider losses on the output of the form
\begin{equation} \label{eq:genreg_lkl}
%\resizebox{0.4\textwidth}{!}{$
    \mathcal{L}(W) = \sum_{i=1}^n h(f(\psi(W \phi(x_i)))) - y_i^\top  f(\psi(W \phi(x_i))),%$}
\end{equation}
where $f, h$ are differentiable functions specified by the desired loss, $y_i \in \mathbb{R}^K$, $x_i \in \mathbb{R}^{d_{in}}$, and $W \in \mathbb{R}^{d_{out} \times d_{in}}$. This class contains logistic regression (with $y$ being a one-hot encoded class vector), least-squares regression, and generalized linear regression---including a neural network with cross entropy loss with one layer being tuned.

We next analyze the gradient of this loss. Our argument is stated with one adapted parameter matrix, but it directly applicable to multilayer and transformer networks with multiple matrices being adapted, where $\phi$, $\psi$, and $f$ will in that scenario vary depending on each parameter matrix's position in the network; $\phi$, $\psi$, and $f$ will depend on other parameter matrices and the current value of their adaptations (by definition of gradients). The interpretation will now be that fixing $A$ when adapting a parameter matrix $W^{(\ell)}$ projects the inputs of the corresponding parameter matrix to a lower-dimensional subspace while retaining the ability to fully match the outputs, and fixing $B$ correspondingly projects the parameter matrix's outputs.

For simplicity of notation, the remaining derivation in this section takes $\phi,\psi$ to be the identity; the extension to general $\phi,\psi$ is clear. 
%and The gradient-based analysis in this subsection focused on adapting only one layer. The results, however, easily extend to adapting multiple layers at once, since partial derivatives decompose. 
%
%
Then, the gradient of \eqref{eq:genreg_lkl} is
\begin{equation}
\label{eq:Wgen}
    \nabla_W  \mathcal{L}(W) = \sum_{i=1}^n J^\top _f(W x_i)\left[\nabla h(f(W x_i)) - y_i\right] x_i^\top  ,
\end{equation}
where $J_f$ is the Jacobian of $f$. % (need to improve this notation).
Starting from this formula, below we incorporate \eqref{eq:Lora} by taking $W = W_0 + B A.$
% and now
% \[
% Y_{targ} = \nabla h(f( (W_0 + \Delta W) X_{targ}).
% \]
% for some unknown $\Delta W$. 

\textbf{Freezing $A$.} Freezing $A = Q$ yields %for the gradient of $B$
\begin{align}\label{eq:Agen}
%\resizebox{0.4\textwidth}{!}{$
\nonumber&\nabla_B  \mathcal{L}(BQ + W_0)=\\& \sum_{i=1}^n\! J^\top _f\!((BQ + W_0) x_i)\left[\nabla h(f((W_0 + BQ) x_i)) \!-\! y_i\right] (Q x_i)^\top. %$}
\end{align}
Like the least-squares case, the input data is projected by $Q$ but the output $y_i$ is unaffected. 


\textbf{Freezing $B$.} Freezing $B = U$ yields %for the gradient of $A$
\begin{align}\label{eq:Bgen}
%\resizebox{0.4\textwidth}{!}{$
\nonumber&\nabla_A  \mathcal{L}(UA + W_0) =\\& U^\top \! \sum_{i=1}^n\! J^\top _f((UA + W_0) x_i)\left[\nabla h(f((W_0 + UA) x_i))\! - \!y_i\right] x_i^\top .%$}
\end{align}
%Note that $J^\top _f((UA + W_0) x_i)\left[\nabla h(f((W_0 + UA) x_i)) \!-\! y_i\right]$ 
Here, the coefficient of $x_i^\top$
can be thought of as the output fit term. It includes the Jacobian of $f$ since $f$ is applied between the weights and the output. Compared to \eqref{eq:Wgen} and \eqref{eq:Agen}, in \eqref{eq:Bgen} this output fit term is projected  by $U$. If $f$ is (near) linear, %i.e., $J_f(\cdot)$ is (approximately) a constant, 
then this projection will be (approximately) data-independent, highlighting the loss of output information when freezing $B$.

Hence, in this more general setting, the different roles of $A$ and $B$ are still apparent, and we expect an asymmetry in being able to fit the output. %To make this more clear, we consider an example.


\textbf{Example: Logistic regression.} For multiclass logistic regression, we have a training dataset $\{(x_i, c_i)\}_{i=1}^n$ where $x_i \in \R^{d}$ (features) and $c_i \in \{1, \dots, K\}$ (label). Denote by $y_i \in \R^{K}$ the vector with $y_{c_i} = 1$ and $y_{k} = 0$ for $k \neq c_i$. The log likelihood is the cross-entropy error
\begin{equation} \label{eq:logreg_lkl}
    \mathcal{L}(w_1, \dots, w_K) = \sum_{i=1}^n \sum_{k=1}^K y_i \ln(p_{i,k}),
\end{equation}
where $p_{i,k} = \frac{\exp(w_k^\top  x_i)}{\sum_{l=1}^K \exp(w_l^\top  x_i)}$ and $w_k \in \R^d$. 
Let $W \in \R^{K \times d}$ whose $k$-th row is $w_k$. Then, \eqref{eq:logreg_lkl} becomes
\begin{align} \label{eq:logreg_lkl_2}
%\resizebox{0.4\textwidth}{!}{$
    \nonumber\mathcal{L}(W) %&= -\sum_{i=1}^n y_i^\top  \ln\left(\frac{e^{W x_i}}{\mathbf{1}^\top  e^{W x_i}}\right) \\&
    = \sum_{i=1}^n  \ln(\mathbf{1}^\top e^{W x_i})  - y_i^\top  W x_i,%$}
\end{align}
where $\mathbf{1}$ is the column vector of size $K$ with all elements equal to 1; note $y_i^\top  \mathbf{1} = 1$ due to the one-hot structure. This loss can be put in the form \eqref{eq:genreg_lkl} by setting 
$f(z) = z$ and $h(z) = \ln(\mathbf{1}^\top e^{z})$. For freezing, we then have 
\begin{align*}
    \nabla_A  \mathcal{L}(UA) &= U^\top  \sum_{i=1}^n (y_i - p_i(UA)) x_i^\top  \qquad\textrm{and}\\
%\end{equation*}
%and 
%\begin{equation*}
    \nabla_B  \mathcal{L}(BQ) &= \sum_{i=1}^n (y_i - p_i(BQ)) (Q x_i)^\top,
\end{align*}
where $p_i(W) =  \frac{e^{W x_i}}{\mathbf{1}^\top  e^{W x_i}} \in \R^K$.
Freezing $B = U$,  as in least-squares, implies that each output $y_i$ is projected as $U^\top  y_i$, implying that, at best, the model can hope to only learn outputs in the small random subspace $U$. In contrast, freezing $A=Q$ is  equivalent to logistic regression on the full output with features projected by $Q$: $\{(Qx_i, y_i)\}_{i=1}^n$. 

%\paragraph{Multilayer extension} 



% {\color{red} 
% \subsection{Effect of layer-wise freezing (temporarily added by Aritra:)}
% In this section, we take a look at how freezing A or B at various layers  may affect the performance of the output. Consider a setting involving L layers. Specifically, let the pretrained linear model covariates $W_0$ be represented as product matricess, i.e., $W_0=\prod_{i=L}^{1} W_{0i}=W_{0L}\ldots W_{01}$. When the low-rank update is performed on the first layer only, the updated model (without the bias term) is:

% \[
% \hat{y}(x) = W_{0L}\ldots(W_{01} + BA) x 
% \]

% In that case the loss function becomes

% \begin{eqnarray}
% \label{eq: loss_product}
% \mathcal{L}(A,B) &= \mathbb{E}_{ X_{targ}} \left\| (W_{targ} - W_{0L}\ldots(W_{01} + BA) ) X_{targ} \right\|_2^2 \nonumber \\
% & \hspace{5 em} + d_{out}\sigma^2 \nonumber\\
% &= \mathbb{E}_{ X_{targ}} \left\| \Delta X_{targ} +(W_{0L}\ldots W_{02}BA ) X_{targ} \right\|_2^2 \nonumber \\
% & \hspace{5 em} + d_{out}\sigma^2,
% \end{eqnarray}
% where $\Delta=W_{0L}\ldots W_{01}- W_{targ}$.

% Assume the pretrained matricesConsider optimizing Eq.~\eqref{eq: loss_product} for 

% {\textbf{orthonormal matrix B frozen:}}

% }
% \subsection{Experimental Illustration}
% We should also have a pictorial graphic probably

% Nonlinear experiments



\subsection{Advantages of tuning only $B$ over $BA$ together}
\label{Advantages of tuning $B$ only over $BA$ together}

In the previous section, we established that fine-tuning $B$ alone is typically superior to fine-tuning $A$ alone. It remains, however, to motivate fine-tuning $B$ alone over fine-tuning both $A$ and $B$ together. In this section, we show that the reduced amount of adapted parameters by (roughly) half provides computational gains and improvements in information-theoretic generalization bounds. 

\subsubsection{Number of parameters} The key benefit of LoRA is parameter efficiency, which saves memory during training, storage and communication \cite{lialin2023scaling}. Fine-tuning $B$ alone as opposed to both $A$ and $B$ reduces the number of parameters by a factor of $\frac{d_{out} }{d_{out} + d_{in}}$, which equals $0.5$ when $d_{in} =d_{out}$. 

\subsubsection{Generalization bounds}

%\textbf{Notation.} Unless otherwise stated, capital letters denote random variables, and lower-case letters indicate their realizations. We c
Consider a learning task, where the training examples lie in $\mathcal{Z} = \mathcal{X} \times \mathcal{Y}$; here, $\mathcal{X}$ denotes the feature space and $\mathcal{Y}$ is the label space. Suppose one observes a training set $S_n \triangleq (Z_1, \dots, Z_n) \in \mathcal{Z}^n$, with $n$ i.i.d.\ training examples from unknown distribution $\mu$. Denote by $\mu^{\otimes n} = \mu \times \dots \times \mu$ the distribution of $S_n$. The objective of the learner is to find a predictor $f : \mathcal{X} \to \mathcal{Y}$ that maps features to their labels. We assume each predictor is parameterized by $w \in \mathcal{W}$ (e.g., if $f$ is a neural network, $w$ denotes its weights). Denote by $\mathcal{A} : \mathcal{Z}^n \to \mathcal{W}$ the learning algorithm which selects a predictor given $S_n$. $\mathcal{A}$ is, in general, a probabilistic mapping, and we denote by $P_{W|S_n}$ the distribution of its output $W$ given input $S_n$. If $\ell : \mathcal{W} \times \mathcal{Z} \to \mathbb{R}_+$ is a loss, we define: %the \emph{population risk} becomes
\begin{align*}
\textrm{Population risk:}\quad &
\mathcal{R}_\mu(w) \triangleq \mathbb{E}_{Z \sim \mu}[\ell(w, Z)]
\\
\textrm{Empirical risk:}\quad &
\widehat{\mathcal{R}}_n(w) \triangleq \frac1n \sum_{i=1}^n \ell(w, Z_i).
\end{align*}
% \begin{equation}\nonumber
%     %\forall w \in \mathcal{W}, \quad 
%     \mathcal{R}_\mu(w) \triangleq \mathbb{E}_{Z \sim \mu}[\ell(w, Z)] \,,
% \end{equation}
% and the \emph{empirical risk} is
% \begin{equation}\nonumber
%     %\forall w \in \mathcal{W}, \quad 
%     \widehat{\mathcal{R}}_n(w) \triangleq \frac1n \sum_{i=1}^n \ell(w, Z_i) \,.
% \end{equation}
The generalization error of $\mathcal{A}$ is 
\begin{equation}
%\resizebox{0.4\textwidth}{!}{$
    \generror{\mu}{\mathcal{A}} \triangleq \mathbb{E}_{(W, S_n) \sim P_{W | S_n} \times \mu^{\otimes n}} [\mathcal{R}_\mu(W) - \widehat{\mathcal{R}}_n(W)] \,.%$}
    \nonumber
\end{equation}
We bound this generalization error using the information-theoretic generalization framework of \citet{xu2017}. 
Consider the following incarnations of fine-tuning algorithms, corresponding to classic LoRA (tuning both $A, B$ matrices), tuning only $B$, and tuning only $A$:
\begin{definition}[Fine-tuning algorithms]
\label{def:alg}
Let $\mathbf{W} = \{W_i\}_{i=1}^L$ be the $L$ parameter matrices of a pretrained model. Let $\mathcal{I}\subseteq \{1,\dots, L\}$ be a specified subset of the parameter matrices to be fine-tuned. Given a fine-tuning training set $S_n$, let $r$ be a chosen rank and suppose each tuned parameter is quantized to $q$ bits. We define the following algorithmic frameworks (other details can be arbitrary) for choosing an adaptation $\mathbf{\Delta W} = \{\Delta_i\}_{i \in \mathcal{I}}$, yielding a fine-tuned $W_{tuned} = \{W_{tuned,i}\}_{i=1}^L$ with $W_{tuned,i} = W_i + \Delta_i$ for $i \in \mathcal{I}$ and $W_{tuned,i} = W_i$ otherwise:
\begin{itemize}
    \item $\mathcal{A}_{BA}$: For each $i \in \mathcal{I}$, constrain $\Delta_i = B_i A_i$ and optimize $\{B_i, A_i\}_{i \in \mathcal{I}}$ to fit the data $S_n$.
    \item $\mathcal{A}_{B}$: For each $i \in \mathcal{I}$, sample $Q_i\in \mathbb{R}^{r \times d^{(i)}_{in}}$ at random, constrain $\Delta_i = B_i Q_i$, and optimize $\{B_i\}_{i \in \mathcal{I}}$ to fit the data $S_n$.
    \item $\mathcal{A}_{A}$: For each $i \in \mathcal{I}$, sample $U_i\in \mathbb{R}^{d_{out}^{(i)} \times r}$ at random, constrain $\Delta_i = U_i A_i$, and optimize $\{A_i\}_{i \in \mathcal{I}}$ to fit the data $S_n$.
\end{itemize}
\end{definition}
We have the following lemma, proved in Appendix \ref{app:IT}:
\begin{lemma}[Generalization bounds on adapting $A$ and/or $B$]
\label{lemm:genbd}
    Consider the algorithms of Definition \ref{def:alg}. Assume that %for all $(\mathbf{W}, \mathbf{b})$, 
$\ell^{\mathbf{W}, \mathbf{b}}(\Delta \mathbf{W}, \widetilde{Z})$ is $\sigma$-sub-Gaussian\footnote{Bounded losses are sub-Gaussian.} under $(\Delta \mathbf{W}, \widetilde{Z}) \sim P_{\Delta \mathbf{W} | \mathbf{W}, \mathbf{b}} \times \mu$.
Then,
\begin{align*}
    | \generror{\mu}{\mathcal{A}_{BA}} | &\leq \sqrt{\frac{{2rq\sigma^2\ln 2}}{n}  \sum_{i\in \mathcal{I}} (d_{in}^{(i)} + d_{out}^{(i)} )},\\
    | \generror{\mu}{\mathcal{A}_{B}} | &\leq \sqrt{\frac{{2rq\sigma^2\ln 2}}{n}  \sum_{i\in \mathcal{I}} d_{out}^{(i)} },\\
    | \generror{\mu}{\mathcal{A}_{A}} | &\leq \sqrt{\frac{{2rq\sigma^2\ln 2}}{n}  \sum_{i\in \mathcal{I}} d_{in}^{(i)}}.
\end{align*}
\end{lemma}
This generalization bound increases with the number of parameters being tuned, which is an increasing function of $r$ and the dimensions of the parameter matrices. Importantly, since tuning just one factor ($A$ or $B$) involves tuning fewer parameters than $A$ and $B$ together, the generalization bound is correspondingly smaller. In the case where the $d_{in}^{(i)} = d_{out}^{(i)}$, the bound for tuning one factor only is a factor of $\sqrt{2}$ smaller than the bound for tuning both factors, implying that the rank $r$ for $\mathcal{A}_B$ could be doubled and have a generalization bound matching that of $\mathcal{A}_{BA}$. 


%\subsection{Bounds on the generalization error of LoRA}

% recall subGaussian

%\justin{missing paragraph:  so what?  interpret the information theoretical bounds above in intuitive language and tell us why they're relevant}

% - (m+n-r)*r
% - Fixed A, update B: r*m
% - Fixed B, update A: r*n
% - Fixed U, V, update Sigma: r^2

% \oca{OOD generalization and relation to domainbed?} \kristjan{We won't discuss OOD gen here. It'll be an extra benefit in the experimental section only.}
% \subsection{Expressive Power of LoRA}

% See \Cref{sec:proofs}.

% \paragraph{Idea:} Compare the test risk of full fine-tuning against PEFT (LoRA and variants), e.g., by bounding the norm of their difference. The goal is to identify when LoRA performs (almost) as well as full fine-tuning, and when it fails to approximately match its performance.

% \paragraph{Strategy:} Start with MLP, then include self-attention layers, then multi-head attention layers.



\subsection{Discussion of theoretical analysis}
\label{theoretical_discussion}
The previous two sections establish two conclusions: (1) Tuning $A$ has limited importance when trying to match a desired output; and (2) Tuning one factor instead of two reduces the number of parameters for the same $r$, while improving generalization bounds and potentially providing memory benefits. 


Given a fixed parameter count and generalization budget, therefore, we can use a larger $r = r_{B}$ when fine-tuning $B$ alone than the $r_{BA}$ that would be used on standard LoRA fine-tuning both $A$ and $B$. This addition provides more expressive power for the same number of parameters without loss of generalization bounds. Hence, when matching parameter or generalization budget, we expect that fine-tuning a rank-$r_B$ $B$ typically improves performance over fine-tuning a rank-$r_{BA}$ $BA$ LoRA adaptation. 
%\jz{Clarify the discussion about budget}
%In the next section, we confirm these expectations empirically. %\justin{seems clear from the title ``experiments'' ;-) }

==> section_05_experiments.tex <==
\section{Experiments}\label{sec:exps}

We investigate the asymmetry of low-rank adaptation methods with RoBERTa~\citep{liu2019roberta}, BART~\citep{Lewis_2020_bart}, 
Llama-2~\citep{touvron2023llama}, and Vistion Transformer~\citep{dosovitskiy2020_ViT}. 
We evaluate the performance of fine-turning strategies on natural language understanding (GLUE~\citep{Wang_2018_glue}, MMLU~\citep{hendrycks2020_mmlu}), natural language generation (XSum~\citep{Narayan_2018_xsum} and CNN/DailyMail~\citep{Chen_2016_cnndailymail}), and multi-domain image classification~\citep{gulrajani2020search}.

%\textbf{Implementation details.}
We implement all algorithms using PyTorch starting from the publicly-available Huggingface Transformers code base~\citep{wolf2019huggingface}. The conventional LoRA method applies a scaling coefficient $\alpha/r$ to $\Delta W$. Following LoRA~\citep{Hu2021LoRALA}, we fix $\alpha=2r$ to be twice the rank.  
Throughout our experiments, we use $\hat{A}$ to indicate matrix $A$ is being updated during fine-tuning and use subscripts \textit{\{rand, $0$, km\}} to indicate that the matrix is initialized as a random orthonormal matrix, zero matrix, and the random uniform initialization used in the original LoRA, respectively. 
Note that a properly normalized $d \times r$ random matrix with independent entries will have close to orthonormal columns when $d \gg r$ (see e.g. Theorem 4.6.1 of~\citet{vershynin2020high_hdp}), implying that the random orthonormal and random uniform initializations should be essentially equivalent. 


We compare to the following methods:
\begin{enumerate}
    \item \textbf{Full fine-tuning (FT):} The most straightforward adaptation method, which initializes model parameters with the pre-trained weights and updates the whole model with gradient back-propagation.
    \item \textbf{Linear Probing (LP)~\citep{kumar2022finetuning}:}  A simple yet effective method that updates the last linear layer.
    \item  \textbf{IA$^3$~\citep{liu2022_ia3}:} Injects learned vectors in the attention and feedforward modules.  
    \item \textbf{LoRA:}~\citep{Hu2021LoRALA} Fine-tunes both $A$ and $B$ matrices of an additive $BA$ adaptation as introduced in previous sections, with a separate adaptation for each query/key/value parameter matrix.
    \item \textbf{AdaLora:}~\citep{zhang2023adalora} A variant of LoRA that adaptively changes the rank for each layer. 
\end{enumerate}

\subsection{Natural Language Understanding}
We use the General Language Understanding Evaluation~\citep[GLUE,][]{Wang_2018_glue} to evaluate the fine-tuning performance of different fine-tuning strategies. The GLUE benchmark contains a wide variety of tasks including question-answering, textual similarity, and sentiment analysis. We applied fine-tuning methods to the RoBERTa (large) model~\citep{liu2019roberta}, which has 355M parameters. To enable a fair comparison, we initialize the weights for all tasks with the original pretrained RoBERTa weights. 


In Table \ref{tab:NLU_all_results} (see the appendix for an expanded table), we compare different freezing \& initialization strategies with LoRA and other baselines. 
We  \underline{underline} to indicate that performance is better than conventional LoRA also we use \textbf{bold} to denote the best performance when freezing one of the matrices. First, we can see a clear trend where solely updating the $B$ matrix outperforms just learning the $A$ matrix. In addition, when doubling the rank to match the trainable parameters,  $\mathbf{\hat{B}}_0 A_{orth}$ consistently outperforms conventional LoRA. This confirms our hypothesis in \S\ref{theoretical_discussion} that any loss in expressive power by not tuning $A$ can be made up for by the larger intrinsic rank of $B$ at no additional parameter cost. In fact, its performance statistically matches that of AdaLoRA, which uses over 3 times the parameters (incurring the associated memory and training costs). % with the same amount of learnable parameters, which agrees with our theoretical analysis in \S \ref{theoretical_discussion}.


% Here, we can see different initialization methods are affecting the performance as discussed in previous studies~\citep{kopiczko2024vera}.

To assess the effects of different initialization methods for low-rank adaptation, we investigate different initialization methods thoroughly in Table \ref{tab:NLU_initialization}.  We can see that the best results always come from orthogonal initialization, which further supports our conclusions in \S\ref{sec:Analysis}. 

\begin{table}[t!]
  \centering
  % \footnotesize
  \addtolength{\tabcolsep}{-4pt}
  
  \caption{  R-1/2/L (\%)
 on text summarization with BART-large on XSum and CNN/DailyMail. 
 %The first two rows indicate the asymmetry of freezing one of the two factors, and the last two rows show the results of tuning both matrices with different initializations, showing that the asymmetry is not explained by the initialization strategy.
  }
  \label{tab:NLG}
  \resizebox{0.5\columnwidth}{!}{%
  \input{tables/text_summarization}}
\end{table}

\begin{table*}[!t] 
\centering
\caption{DomainBed results (mean accuracy and standard deviation in $\%$). ID and OOD denote in-domain and out-of-domain test error, respectively. For OOD we report the average performance across different environments.
}
\resizebox{1.75\columnwidth}{!}{%
  \input{tables/domainbed_new}}
\label{tab:domainbed_new}
\end{table*}

 \begin{table}[t!]
  \centering
  % \footnotesize
  \addtolength{\tabcolsep}{-4pt}
  
  \caption{ Accuracy (\%) on MMLU benchmark. 
  }
  \label{tab:mmlu}
  \resizebox{0.9\columnwidth}{!}{%
  \input{tables/mmlu_table}}
\end{table}

\subsection{Natural Language Generation}
To investigate the asymmetry of low-rank fine-tuning in natural language generation (NLG), we fine-tune a BART-large model~\citep{Lewis_2020_bart} and evaluate model performance on the XSum~\citep{Narayan_2018_xsum} and CNN/DailyMail~\citep{Chen_2016_cnndailymail} datasets. Following \citet{zhang2023adalora}, we apply low-rank adaptation to every {query/key/value} matrix and report ROUGE 1/2/L scores (R-1/2/L,~\citep{lin2004rouge}). We fine-tune models for $15$ epochs. We select the beam length as $8$ and batch size as {$48$} for XSum, and the beam length as $4$, batch size as {$48$} for CNN/DailyMail. More details of the configurations are in the Appendix \ref{appendix:text-summarization}. 

The results are summarized in Table \ref{tab:NLG}. In the first two rows, we observe the asymmetry between the factors since freezing $A$ and only updating $B$ always outperforms only updating $A$. The last two rows show the results of tuning both matrices with different initializations, showing that the asymmetry is not explained by the initialization strategy.



\subsection{Massive Multitask Language Understanding}
We fine-tune the pretrained Llama-2-7B model~\citep{touvron2023llama} using instruction tuning on the Alpaca dataset~\citep{wang2023far_alpaca}. We assess the asymmetry on the MMLU benchmark~\citep{hendrycks2020_mmlu}, which consists of 57 distinct language tasks. As shown in Table \ref{tab:mmlu}, the asymmetry also exists in larger language models, and updating $B$ consistently outperforms updating $A$. Moreover, it also outperforms standard LoRA except for ``Other'' where it matches the performance, reflecting the benefits of being able to increase $r$ without tuning more parameters. 




% \rickard{I believe reviewers might comment on the decision to use MMLU in this setting rather than some of the datasets more widely used in other LoRA papers. In addition, I think domain-bed is good for showing domain adaption, but if the aim is to show performance on vision data (as a modality), people might think it is an odd choice -- a larger more widely used vision dataset might be more suitable in that case.}
% \oca{Would be good to add larger vision datasets if we have time :) But the main point of domainbed is that only updating B behaves differently based on whether we are generalizing in domain or out of domain. I still need to run the experiments but the main observation is that tuning both B and A works best in-distribution and tuning only B becomes substantially better for out of distribution generalization}



 

% \begin{table*}[h]
% \centering
% \caption{DomainBed results (mean accuracy and standard deviation in $\%$). ID and OOD denote in-domain and out-of-domain generalization, respectively. $\hat{(\cdot)}$ means the matrix is trained, while $(\cdot)_{rand}$ means it is randomly initialized and frozen. $r$ stands for rank.}
% \resizebox{2.2\columnwidth}{!}{%
%   \input{tables/domainbed}}
% \label{tab:domainbed}
% \end{table*}



\subsection{Vision Transformers and Generalization}

We next measure generalization, motivated by the theory in \S\ref{Advantages of tuning $B$ only over $BA$ together}. In particular, we work with ViTs in image classification tasks using the Domainbed testbed for domain generalization~\cite{gulrajani2020search}. Domainbed contains several datasets, each composed of multiple environments (or domains). Classes in each environment tend to be similar at a high level but differ in terms of style. We fine-tune a pre-trained ViT, originally trained on ImageNet, on the LabelMe, Cartoon, and Clipart environments within the VLCS, PACS, and Office-Home datasets, respectively. We employ different benchmark fine-tuning methods such as full fine-tuning, linear probing, and LoRA, and compare their performance to freezing either $A$ or $B$ in in-domain and out-of-domain generalization. We adhere to the original $80\%$ training and $20\%$ testing splits. 

Results are presented in Table~\ref{tab:domainbed_new}. In line with our expectations, randomly initializing and freezing matrix $A$ while only updating matrix $B$ generally results in better out-of-domain test accuracy. We report additional generalization results in Appendix~\ref{Additional Domainbed results}, in which we compare the train set and test set accuracy of the different approaches. We consistently find that fine-tuning a single matrix leads to smaller gaps between these two quantities compared to LoRA, paralleling the corresponding reduction in the generalization bounds of \S\ref{Advantages of tuning $B$ only over $BA$ together}.


% \subsection{Ablation study and analysis}


==> tables/glue_table_2_full.tex <==
\begin{tabular}{l|c|ccccccccc}
  \hline
  \toprule
  Model \& Method & \# Trainable & \multicolumn{8}{c}{} \\
         & Parameters & MNLI & SST-2 & MRPC & CoLA & QNLI & RTE & STS-B & Avg. \\
  \midrule
  
  \midrule 

  $\hat{B}_0 \hat{A}_{V}$  & 0.8M & 90.4\textsubscript{$\pm$0.11} & 95.9\textsubscript{$\pm$0.16}  & 90.7\textsubscript{$\pm$0.84} & 64.0\textsubscript{$\pm$0.50} & 94.4\textsubscript{$\pm$0.16} &  {84.1}\textsubscript{$\pm$0.15} & 91.8\textsubscript{$\pm$00.15} &  \\
  
  $\hat{B}_0 \hat{A}_{rand}$  & 0.8M & 90.4\textsubscript{$\pm$0.15} & 96.0\textsubscript{$\pm$0.11} & 91.5\textsubscript{$\pm$1.1} & 64.1\textsubscript{$\pm$0.67} & 94.5\textsubscript{$\pm$0.11} &  \textbf{85.6}\textsubscript{$\pm$0.96} & \textbf{92.0}\textsubscript{$\pm$0.31} &  \\
  
  $\hat{B}_0 \hat{A}_{km}$ (LoRA)  & 0.8M & 90.3\textsubscript{$\pm$0.07} & 95.6\textsubscript{$\pm$0.36} & 90.3\textsubscript{$\pm$0.85} & 64.4\textsubscript{$\pm$1.8} & 94.0\textsubscript{$\pm$0.29} &  {84.1}\textsubscript{$\pm$0.96} & 91.5\textsubscript{$\pm$0.16} & \\
  
  $\hat{B}_U \hat{A}_0$ & 0.8M & 90.3\textsubscript{$\pm$0.07} & \textbf{96.1}\textsubscript{$\pm$.18} & \textbf{91.7}\textsubscript{$\pm$0.33} & 64.9\textsubscript{$\pm$1.5}  & \textbf{94.7}\textsubscript{$\pm$0.33}  &  {84.8}\textsubscript{$\pm$0.96} & 91.9\textsubscript{$\pm$0.19} & \\
  
  $\hat{B}_{rand} \hat{A}_0$  & 0.8M & 90.3\textsubscript{$\pm$0.27}  & 96.0\textsubscript{$\pm$.26} & 90.8\textsubscript{$\pm$0.51} & \textbf{66.0}\textsubscript{$\pm$1.01} & 94.5\textsubscript{$\pm$0.38} &  {83.6}\textsubscript{$\pm$1.5} & \textbf{92.0}\textsubscript{$\pm$0.18}  &   \\
  
  $\hat{B}_{km} \hat{A}_0$  & 0.8M & 35.5\textsubscript{$\pm$1.6} & 95.6\textsubscript{$\pm$.65} & 90.0\textsubscript{$\pm$0.46} & 21.3\textsubscript{$\pm$36.} & 93.8\textsubscript{$\pm$0.01} &  {57.4}\textsubscript{$\pm$0.17} & 91.6\textsubscript{$\pm$0.43} &  \\
  
  \bottomrule
  \end{tabular}
